Path Planning for Concentric Tube Robots: a Toolchain with Application to Stereotactic Neurosurgery

We present a toolchain for solving path planning problems for concentric tube robots through obstacle fields. First, ellipsoidal sets representing the target area and obstacles are constructed from labelled point clouds. Then, the nonlinear and highly nonconvex optimal control problem is solved by introducing a homotopy on the obstacle positions where at one extreme of the parameter the obstacles are removed from the operating space, and at the other extreme they are located at their intended positions. We present a detailed example (with more than a thousand obstacles) from stereotactic neurosurgery with real-world data obtained from labelled MPRI scans.

==> inc/05_numerics.tex <==
\section{Numerics}\label{sec:numerics}

\red 
The labelling of these areas was done by medical professionals on MRI scans.

WE: I think it is maybe enough to just mention that you use quaternions to represent rotation matrices in the numerics, because... reason...?

Full details of the example so that it is reproducible by someone else...

change $\R^0$ to quaternions... \begin{align*}
	\R^0(\boldsymbol{q}) = \begin{bmatrix}
		1 - 2(q_2^2-q_3^2) & 2(q_1 q_2 - q_0 q_3) & 2(q_1 q_3 + q_0 q_2)\\
		2(q_1 q_2 + q_0 q_3) & 1 - 2(q_1^2-q_3^2)  & 2(q_2 q_3 - q_0 q_1)\\
		2(q_1 q_3 - q_0 q_2) & 2(q_2 q_3 + q_0 q_1) & 1 - 2(q_1^2-q_2^2)
	\end{bmatrix}
\end{align*}\blk







==> inc/06_discussion.tex <==
\section{Discussion and Perspectives}

The numerical results demonstrate how homotopy methods



We made use of a number of heurtistics...

The numerical results showcase the strength of homotopy methods to solve optimal control problems. 

The approach is not guaranteed to converge, and we have examples like this... this happens when a solution is not found for some lambda.

Topology changes are not addressed yet.

We get local solutions, (which are still valuable).

There are better ways to update lamba...
